Infinite towers in the graph of a dynamical system

Chaotic attractors, chaotic saddles and periodic orbits are examples of chain-recurrent sets. Using arbitrary small controls, a trajectory starting from any point in a chain-recurrent set can be steered to any other in that set. The qualitative behavior of a dynamical system can be encapsulated in a graph. Its nodes are chain-recurrent sets. There is an edge from node A to node B if, using arbitrary small controls, a trajectory starting from any point of A can be steered to any point of B. We discuss physical systems that have infinitely many disjoint coexisting nodes. Such infinite collections can occur for many carefully chosen parameter values. The logistic map is such a system, as we showed in arXiv:2008.08338. To illustrate these very common phenomena, we compare the Lorenz system and the logistic map and we show how extremely similar their bifurcation diagrams are in some parameter ranges.

==> figLMBDnew.tex <==
\begin{figure}
 \centering
 \includegraphics[width=12cm]{cr3.png}
  \caption{{\bf Bifurcation diagram and sample graphs of the logistic map.} 
%   The logistic map has a top node, the point 0, that for simplicity is not shown.
  This picture shows the bifurcation diagram of the logistic map in the range of parameter values $[2.9,4]$.
  For each value of $\mu$, the attracting set is painted in shades of gray, depending on the density of the attractor, repelling periodic orbits in green and repelling Cantor sets in red. Below the $\mu$ axis we show seven samples of the graphs illustrating some of the possible variability. In these graphs, each colored disk is a node. Each black disk represents an attractor, each green disk represents a repelling periodic orbit and red represents a chaotic Cantor set repellor. For simplicity we always omit the top node, which is the point 0. Graph T4 represents the infinite tower at the first Feigenbaum point. It has infinitely many unstable periodic orbit nodes.
  }
  \label{fig:full}
\end{figure}

%%%%%%%%%%%%%%%

\begin{figure}
 \centering
 \includegraphics[width=13cm]{crsmall}
 \caption{{\bf Towers of nodes shown below the period-3 window of the logistic map bifurcation diagram.}
    This figure is a blow-up from Fig.~\ref{fig:full}, and uses the color-coding from that figure. Graph T8 has two levels of nodes that are Cantor sets repellors and the second is painted in blue.
 %The period-3 window of the logistic map starts at and ends at ...
 %$\mu\INT$ (\ref{muInt}).
 %=1.5[ 1 + (19-3\sqrt{33})^{1/3} + (19+3\sqrt{33})^{1/3} ]\simeq3.67857$,
% The black dots on the $\mu$ axis are sample values sampling some of the possible towers near the value where the period three orbit first appears, $\mu = 1+\sqrt 8\simeq3.8284$.
%Red nodes denote fractal chaotic saddles. Blue and green nodes are periodic orbits. Black denotes attracting sets which occur at the bottom of the tower. 
In the bifurcation diagram, the chain recurrent sets have the same coloring as their nodes. 
Graph T5 represents the infinite tower at the first Feigenbaum point of the main cascade of the period-3 window. 
%It has infinitely many unstable periodic orbit nodes.
%Notice that we do not include in the pictures of the towers the zero node, which is always on top.
}
 \label{fig:p3}
\end{figure} 
%%%%%%%%%%%%%%%


==> figLogisticBD.tex <==
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{lm}
 \caption{{\bf The Bifurcation Diagram of the Logistic Map.} To the left of the Feigenbaum-Myrberg parameter value $\mu_{FM}\simeq3.56994567$, we see the well-known period-doubling cascade. To its right, we see lots of chaos but also many windows, \ie, intervals in parameter space that begin with a periodic attractor which evolves through period-doubling into small intervals of chaos. This picture is created by plotting trajectories. More frequently visited regions are darker. Points on attracting periodic orbits of period less than 26 are indicated by black dots. Notice, in particular, that many of these points are near where $x=0.5$. In colors are highlighted, besides $\mu_{FM}$, the largest period-6 window, the intersection parameter value $\mu\INT=1.5[ 1 + (19-3\sqrt{33})^{1/3} + (19+3\sqrt{33})^{1/3} ]\simeq3.67857$, the largest period-5 window and the largest period-3 window. Notice that many high-density lines intersect at $(\mu\INT,x\INT)$ (see figure). Each of the high-density lines is the image of the $x=0.5$ line under $\ell^n_\mu$ for some $n$. In the bottom right box it is shown a detail of the cascade about $x=0.5$ inside the period-5 window.
 }
 \label{fig:lmbd}
\end{figure} 
%%%%%


==> figLorenzCR.tex <==
\begin{figure}
 \centering
 \includegraphics[width=12.5cm]{l5}
 \caption{{\bf A periodic window in the bifurcation diagram of the Poincar\'e map of the Lorenz system}.
 This figure is placed here for comparison with the very similar Fig.~\ref{fig:p3} for the logistic map. 
 More information about the Lorenz system and its Poincar\'e map is given in the text.
 This window runs from $\rhoo\simeq208.520$ to $\rhoo\simeq209.453$. 
 There is a rectangle in the right side of Fig.~\ref{fig:lfull}(top) that represents the area shown here. There one can see that the red Cantor set and the attractor have components for $y$ outside of the range shown here and there is another attractor. 
 Several nodes that are unstable Cantor sets are shown in red and blue. 
}
 \label{fig:lcr}
\end{figure} 

==> figLorenzPeriod4.tex <==
\begin{figure}
 \centering
 \includegraphics[width=12cm]{l2}
 \caption{{\bf Bifurcation Diagram}. This is a detail, in the $(\rho,y)$ projection, of the large period-4 window of the bifurcation diagram of the Lorenz system. The window starts at $\rho\simeq142.26$ and ends at $\rho\simeq162.12$.}
 \label{fig:l2}
\end{figure} 

==> figs.tex <==
%%%%%%%%%%%%%%%
\newpage
\begin{figure}
 \centering
 \includegraphics[width=12.21cm,height=6cm]{l1}\\
 \includegraphics[width=12cm,height=6cm]{l1x}\\
 \includegraphics[width=12cm,height=6cm]{l1a}\\
 \caption{{\bf Bifurcation Diagram}. These are the projections onto the $(\rho,y)$ (Top panel) and $(\rho,x)$ (Bottom panel) planes of the bifurcation diagram for the Poincar\'e Return map of the Lorenz equations~(\ref{eq:Lor}) using the plane $\Pi$ defined by $z=\rho-1$. A dot is plotted in the $(\rho,y)$ (resp. $(\rho,x)$) plane when a trajectory crosses downward past $\Pi$ through the point $(x,y,\rho-1)$. The regions where there is speckled white and magenta dots is where the attractor is low density. The Lorenz attractor typically has great variations in density, so extremely long trajectories would be needed to reveal such parts of the attractor.
 }
 \label{fig:l1}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{l2}
 \caption{{\bf Bifurcation Diagram}. This is a detail, in the $(\rho,y)$ projection, of the large period-4 window of the bifurcation diagram of the Lorenz system. The window starts at $\rho\simeq142.26$ and ends at $\rho\simeq162.12$.}
 \label{fig:l2}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{l3.png}
 \caption{{\bf Bifurcation Diagram}. This is a detail, in the $(\rho,y)$ projection, of the upper cascade of the main period-4 window of the bifurcation diagram for the Poincar\'e Return map of the Lorenz system.}
 \label{fig:l3}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{l4}
 \caption{{\bf Bifurcation Diagram}. This is a detail, in the $(\rho,y)$ projection, of the middle cascade in the main period-3 window of the upper cascade in the main period-4 window (Fig.~\ref{fig:l3}) of the bifurcation diagram for the Poincar\'e Return map of the Lorenz system (Fig.~\ref{fig:l1}).}
 \label{fig:l4}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{l5}
 \caption{{\bf Bifurcation Diagram}. This picture shows the attractor (in black/gray) and the rest of the chain-recurrent set (in red and blue) in the largest period-3 window of the Lorenz system bifurcation diagram. The window starts at about $\rho=208.520$ and ends at about $\rho=209.453$.}
 \label{fig:l5}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{l6.png}
 \caption{{\bf The Lorenz Poincare return map for $\rho=209.2$, which has a period-3 attractor}. A period-3 attractor is shown with black dots on the blue curve. The blue curve is a global attractor for the $(x,y)$ region shown. The region in white are points that are attracted to another attractor, that is off-screen. The blue curve includes the period-3 attractor and a chain-recurrent Cantor set of saddle points and the unstable manifolds of all of the periodic orbits in the Cantor set. Almost all points in the colored region are in the basin of attraction of the period-3 orbit. Yellow indicates rapid convergence to the period-3 orbit, while red indicates slow convergence. Red points are close to points that are attracted to the Cantor set on the blue line.}
 \label{fig:l6}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=5cm]{lorenzOrbit-r208-tf5000-dT11.png} \includegraphics[width=5cm]{lorenzOrbit-r209_2-tf5000-dT11.png}
 \caption{{\bf Attractors of the Poincar\'e Map of the Lorenz system.}. This picture shows two attractors of the Lorenz system for $\rho=208$ (left) and $\rho=209$ (right) together with the plane $z=\rho-1$. The plane is translucent so that it is possible to see also the portion of the attractor on the other side (shaded in blue). The intersections of the attractor with the plane $z=\rho-1$ is shown in Fig.~\ref{fig:l7} for several values of $\rho$. }
 \label{fig:l7}
\end{figure} 
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=11.8cm]{la.png}
 \caption{{\bf Attractors of the Poincar\'e Map of the Lorenz system.} The pictures above show the attractor of the Poincar\'e map of the Lorenz system  in the $(x,y)$ plane for five different values of $\rho$. In all pictures $x$ ranges from $-20$ to $20$ and $y$ ranges from $-100$ to $100$. Each panel is the plot of a single trajectory, Hence low density regions of the attractor may not be represented.
 }
 \label{fig:la}
\end{figure} 
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{lm}
 \caption{{\bf Bifurcation Diagram}. This is the bifurcation diagram of the Logistic map}
 \label{fig:lmbd}
\end{figure} 
%%%%%
\begin{figure}
 \centering
 \includegraphics[width=12cm]{cr3.png}
  \caption{{\bf \allblue The bifurcations diagram and sample graphs of the logistic map.} 
  The logistic map has a top node, the point 0, that for simplicity is not shown.
  For each value of $\mu$, the attracting set is painted in gray or black, depending on the density of the attractor, repelling periodic orbits in green, and repelling Cantor sets in red. 
  \allred WE NEED TO DISCUSS THE T$_J$ GRAPHS SOMEPLACE.
  }
  \label{fig:full}
\end{figure}

%%%%%%%%%%%%%%%
\begin{figure}
 \centering
 \includegraphics[width=13cm]{crsmall}
 \caption{{\bf Towers of nodes, \ie, chain recurrent sets, in the Logistic map diagram.}
 \allblue
 The black dots on the $\mu$ axis are sample values sampling some of the possible towers near the value where the period three orbit first appears, $\mu = 1+\sqrt 8\simeq3.8284$.
Red nodes denote fractal chaotic saddles. Blue and green nodes are periodic orbits. Black denotes attracting sets which occur at the bottom of the tower. 
In the bifurcation diagram, the chain recurrent sets have the same coloring as their nodes. Notice that we do not include in the pictures of the towers the zero node, which is always on top.}
 \label{fig:p3}
\end{figure} 
%%%%%%%%%%%%%%%


